Revisiting Text-to-Image Evaluation with Gecko: On Metrics, Prompts, and Human Ratings

While text-to-image (T2I) generative models have become ubiquitous, they do not necessarily generate images that align with a given prompt. While previous work has evaluated T2I alignment by proposing metrics, benchmarks, and templates for collecting human judgements, the quality of these components is not systematically measured. Human-rated prompt sets are generally small and the reliability of the ratings -- and thereby the prompt set used to compare models -- is not evaluated. We address this gap by performing an extensive study evaluating auto-eval metrics and human templates. We provide three main contributions: (1) We introduce a comprehensive skills-based benchmark that can discriminate models across different human templates. This skills-based benchmark categorises prompts into sub-skills, allowing a practitioner to pinpoint not only which skills are challenging, but at what level of complexity a skill becomes challenging. (2) We gather human ratings across four templates and four T2I models for a total of >100K annotations. This allows us to understand where differences arise due to inherent ambiguity in the prompt and where they arise due to differences in metric and model quality. (3) Finally, we introduce a new QA-based auto-eval metric that is better correlated with human ratings than existing metrics for our new dataset, across different human templates, and on TIFA160.

==> 05-human-data-20240917-1821.tex <==
\section{Collecting Human Judgements}
\label{sec:humanjudgement}

When evaluating T2I models, existing work uses different \emph{annotation templates} for collecting human judgements. 
While human annotation is the gold-standard for evaluating generative models, previous work shows the design of a template and background of annotators can significantly impact the results \citep{clark-etal-2021-thats}.
  
%
We examine differences between templates and how the choice of a template \citep{cho2023davidsonian,liang2023rich} impacts the outcomes when comparing four models: SD1.5 \citep{rombach2022high}, SDXL \citep{podell2023sdxl}, Muse \citep{chang2023muse}, and Imagen Vermeer \citep{vasconcelos2024greedygrowingenableshighresolution}. Muse is based on the original model, but trained on other data sources.
We find that the template {\em does impact results} when comparing raw scores for both inter-annotator agreement and, more importantly, model ordering in terms of average score. % Cf Table 3, model ordering for each metric can be different. 
We further introduce a principled method to determine model ordering based on human judgements and {\em again} find that the template still impacts the results. We consider three \emph{absolute} comparison templates (Likert, Word Level, and DSG(H)) which evaluate models individually, and a template for \emph{relative comparison} (side-by-side, SxS). The templates are defined below and a high-level visualisation of each template is in panel (b) of \Figure{fig:overview}. Extensive information about the templates can be found in \Appendix{app:human_eval_templates}.


\subsection{Comparing Annotation Templates}

Before further exploring how human judgements impact results, we first validate the reliability of each absolute comparison template by measuring inter-annotator agreement. We want to answer the following questions: (1) does the choice of the template impact the quality of the data we can collect; (2) do judgements arising from different templates agree or disagree with each other; (3) is there a subset of prompts which lead to higher agreement among prompts?

%
{\bf Absolute comparison templates.} We collect the human scores on images generated by generative models, and compute  {\bf inter-annotator  agreement}  for  each generative model on different human  evaluation  templates. The agreement is measured by computing the  Krippendorff’s $\alpha$ \citep{hayes2007answering} between ratings from different annotators. Results are reported in Table \ref{tab:h_eval_krippendorff_avg_std}. Krippendorff's $\alpha$ assumes values between -1 and 1, with 1 indicating perfect agreement and 0 chance level \citep{zapf2016measuring}.
%, with 0 indicating no agreement beyond chance levels, 1 perfect agreement, and -1 perfect disagreement \cite{zapf2016measuring}. 
As our goal is evaluating agreement between annotators, in this experiment we keep all \emph{Unsure} ratings, but for the following experiments we pre-process the annotations by removing all such ratings so as to only reflect cases where annotators were confident.
We observe that all human annotators yield agreement on most templates, where the agreements are above chance levels for all generative models, with $\alpha>0.5$, except for the  Likert--SD1.5 pair for Gecko(R). 
We also observe that for Gecko(R), WL is a more reliable template but for synthetic prompts, DSG(H) has higher agreement. 

 We then investigate which templates agree/disagree more with each other {\bf (inter-template correlation)} by computing Spearman's rank and Pearson correlations between scores from each template. Results are in \Appendix{app:human_eval_add_results} and show that there is an overall high correlation between all templates on both Gecko(S)/(R) and the strongest observed correlation among all models and metrics is between the finer-grained templates, WL and DSG(H), on Gecko(S).
\begin{mdframed}[style=mystyle]
{\bf Takeaway:} While all templates yield in general above chance inter-annotator agreement, fine-grained templates, WL and DSG(H) yield the highest agreement, and the fine-grained templates (WL and DSG(H)) also have the highest inter-template correlation.
\end{mdframed}

%\olivia{Should we bring results for SxS here too?}
%\isabela{If we bring SxS results for consistency with other metrics, I think we should also bring the correlation results across metrics, which might take too much space.}


\noindent {\bf SxS comparison.}
\label{sec:experiments_sxs}
To compare the SxS template with the absolute comparison ones, we compute the accuracy obtained by each absolute template when predicting the preferred model given by SxS annotations with the reliable subsets of both Gecko(R) and Gecko(S). For Gecko(R), we find that DSG(H) presented the best accuracy in 4 out of 6 evaluations, followed by Likert which was the most accurate absolute template in the remaining 2 evaluations. On the other hand, for Gecko(S), we find that WL and Likert predict SxS judgements with higher accuracy, each one being the most accurate template in 3 out of 6 cases, indicating that, overall, Likert scores were able to better predict results of SxS comparisons. The complete set of results is in App. \ref{app:human_eval_add_results}. 
\begin{mdframed}[style=mystyle]
{\bf Takeaway:} While no one absolute template perfectly predicts SxS results, they all perform similarly (71\% on average).
\end{mdframed}

%\olivia{Should we bring results for SxS here too?}\isabela{TODO: discuss which SxS results we will bring to the main text. What should we move from main text to appendix to open up space? Summarise related work and add to the appendix an extended version of it; move Figure 3 and Table 2? }

\input{tables/human_eval_model_comparison.tex}

%\noindent {\bf Sources of disagreement between templates.}
%\olivia{It is unclear why templates seem to give different results: here we analyse qualitatively the areas where we found the largest different between templates and found the following properties which we hypothesise are the sources of this differences. Bring in results from Appendix D.3.}

%\isabela{Appendix D.3 results explain why raters disagree/agree, but it is not clear to me how those results will shed light on the sources of disagreement across templates.}

\begin{mdframed}[style=mystyle]
{\bf Takeaway 4:} Both prompts and templates lead to variance in annotation. The prompt may be ambiguous, contain niche concepts, or ill defined but the template may also have errors, be ambiguous or uncalibrated.
\end{mdframed}

\noindent {\bf Reliable Prompts.}
\label{sec:experiments_reliable}
As we found that differences in human ratings could arise from ambiguity in the prompt such as cases where the prompts contain culturally specific words as \textit{'a bottle of Irn-Bru is sitting on a shelf'}. Here we explore if we can obtain a subset of prompts that are reliably rated---we name these `reliable prompts'.
To evaluate `reliability', we use the extent to which the annotators agree in their ratings regardless of the annotation template and the model used to generate images.
%
To get a set of \emph{reliable prompts}, for each model--template pair, we select the prompts for which inter-rater \emph{disagreement}\footnote{Defined as the variance across the scores given by each rater in the case of Likert, and the average variance across words and questions scores in the case of WL and DSG(H), respectively.} is below 50\% the maximum \emph{disagreement} observed across all prompts for that model--template pair. We then repeat this step for all model--template pairs, and consider the intersection of prompts across these settings as the \emph{reliable prompts}. We further refine this set by removing instances for which all ratings from the Likert template are \emph{Unsure}. This procedure yields a total of 531 and 725 \emph{reliable prompts} for Gecko(R) and Gecko(S), respectively. As we only consider ratings from the absolute comparison templates when finding \emph{reliable prompts}, we investigate how the SxS template agreement (\ie, Krippendorff's $\alpha$) changes given this set. This experiment validates our notion of reliability by evaluating if it is transferable to other templates.  For Gecko(R), we find that using reliable prompts increases the average Krippendorff's $\alpha$ from 0.45 to 0.47, and for Gecko(S) from 0.49 to 0.54, showing that both sets of reliable prompts generalise to other templates. Detailed results are in \Appendix{app:human_eval_add_results}.
\begin{mdframed}[style=mystyle]
{\bf Takeaway 5:} The notion of reliable prompts is useful to get a subset of prompts that lead to higher annotation reliability.
\end{mdframed}


\subsection{Comparing T2I Models}\label{sec:human_eval_comparing_models}

{\bf Setup.} Now we analyse how the choice of annotation template impacts the found model ordering. For the absolute comparison templates, we show in \Table{tab:h_eval_krippendorff_avg_std} the average and standard deviation of all ratings. We verify the significance of outcomes by performing the Wilcoxon signed-rank test for all pairs of models with $p<0.001$. Where results indicate the null-hypothesis is rejected (\ie, the distribution of ratings is significantly different), we can say there is enough evidence that one model is better than another. To determine which model is best, we compare the mean values of their scores. For the SxS template, a model was deem as a better than another if the number of times its was preferred is both higher than for the competitor model and the number of \emph{Unsure} ratings. 

{\bf Results.} \Figure{fig:h_eval_wilcoxon} presents the results for the comparisons between all pairs of models with reliable (Gecko(*)-rel) prompt subsets. We see that Muse is not worse than any of the contenders across all templates and prompt sets; we determine it is the best overall model given human judgement. Also, SD1.5 is worse or the same as other models except for Imagen when evaluated with Gecko(R)-rel.
\Figure{fig:h_eval_wilcoxon} results also shed light on the agreement between templates: for Gecko(S)-rel all templates agree with each other, and for Gecko2K-rel all templates agree or do not contradict each other (\ie, one is significant, the other not) \isabela{Potentially update this once G2K results for SxS are in}. However, for G(R)-rel there is some contradiction, leading to our next finding: 
\begin{mdframed}[style=mystyle]
{\bf Takeaway 6:} The prompt set impacts whether we find agreement between different human annotation templates, but we can find comprehensive sets that do give consistent orderings and thereby more confidence in model rankings.
\end{mdframed}

\input{./tables/human_eval_model_comparison_full}

\noindent{\bf Results by sub skill.} As we have labelled our dataset with skills, we can further explore how human judgements vary by skill and template. Average scores for each template are shown in \Figure{fig:results_by_category_mean_likert} to \Figure{fig:results_by_category_mean_dsg_color}. An interesting observation is that Likert and SxS {\em do not} distinguish much between `easy' and `difficult' skills. However, DSG(H) and WL make this more apparent. For example, we can clearly see that counting and language complexity / compositionality are more challenging with those setups but this is not so obvious under Likert (SxS gives no notion of difficulty).



\noindent {\bf Summary.} We see that our discriminative prompt set, Gecko(S), results in consistent model rankings, independent of the template used. For prompts that test for aspects other than image--text alignment, \ie, Gecko(R), the choice of the annotation template impacts the ordering of the models, but the best and worst models are mostly consistent across templates. In terms of templates, the finer-grained ones (WL and DSG(H)) have better inter-annotator agreement in comparison to Likert and SxS. We also notice that when comparing model rankings with Gecko(R)-rel, DSG(H) is the template that mostly disagrees with the others. \olivia{Not clear this is true anymore.} This finding, along with the higher inter-annotator agreement shown by the WL template, makes it the overall best choice for evaluating image--text alignment on Gecko2K.    


==> tables/correlation_both_modalities.tex <==
% \begin{table}[t]
% \renewcommand{\arraystretch}{1.1}
% \setlength{\tabcolsep}{3pt}

% \centering

% % \begin{subtable}{.8\linewidth}

% % \begin{tabular}{cc}
% %     \begin{minipage}{.7\textwidth}
%     \parbox{.7\textwidth}{
% \resizebox{0.7\textwidth}{!}{%
% \begin{tabular}{c|c|cccc|cccc}
% \hline
%                                   &                                       & \multicolumn{4}{c|}{\textbf{Gecko(R)}}                                                                                                     & \multicolumn{4}{c}{\textbf{Gecko(S)}}                                                                                                                                                                                                                                           \\ \cline{3-10} 
%                                   &                                       & WL                          & Likert                      & \multicolumn{1}{c|}{DSG(H)}                      & SxS                         & WL                          & Likert                               & \multicolumn{1}{c|}{DSG(H)}                               & SxS      \\ \cline{3-10} 
% \multirow{-3}{*}{\textbf{Metrics}} & \multirow{-3}{*}{\textbf{Zero-shot}} & \multicolumn{3}{c|}{SpearmanR}                                                                               & Acc                         & \multicolumn{3}{c|}{SpearmanR}                                                                                                 & Acc              \\ \hline
% {\em Interpretable (QA/VQA)} & & & & \multicolumn{1}{c|}{} & & & & \multicolumn{1}{c|}{} \\
% TIFA$_{\texttt{PALM-2/PALI}}$                                & {\color{ForestGreen}\cmark}                                 & 0.26                        & 0.34                        & \multicolumn{1}{c|}{0.28}                        & 41.7                        & 0.39                        & 0.32                                 & \multicolumn{1}{c|}{0.39}                                 & 53.2                             \\
% DSG$_{\texttt{PALM-2/PALI}}$                              & {\color{ForestGreen}\cmark}                                 & 0.35                        & 0.47                        & \multicolumn{1}{c|}{0.42}                        & 49.6                        & 0.45                        & 0.45                                 & \multicolumn{1}{c|}{{0.45}}                        & 58.1                                   \\ 
% Gecko$_{\texttt{PALM-2/PALI}}$                              & {\color{ForestGreen}\cmark}                                 & \underline{0.41}               & \underline{0.55}               & \multicolumn{1}{c|}{\underline{0.46}}               & \underline{62.1}                        & \underline{0.47}               & \underline{0.52}                        & \multicolumn{1}{c|}{\underline{0.45}}                        & \underline{74.6}                        \\ \hline
% Gecko$_{\texttt{Gemini Flash}}$                      & {\color{ForestGreen}\cmark}                                 & \underline{\textbf{0.43}}               & \underline{\textbf{0.58}}               & \multicolumn{1}{c|}{\underline{\textbf{0.48}}}               & \underline{72.2}                        & \underline{\textbf{0.54}}               & \underline{\textbf{0.59}}                        & \multicolumn{1}{c|}{\underline{\textbf{0.56}}}                        & \underline{\textbf{78.8}}       \\ \hline
% {\em Uninterpretable (single score)} & & & & \multicolumn{1}{c|}{} & & & & \multicolumn{1}{c|}{} \\

% CLIP                               & {\color{ForestGreen}\cmark}                                 & 0.14                        & 0.16                        & \multicolumn{1}{c|}{0.13}                        & 54.4                        & 0.25                        & 0.18                                 & \multicolumn{1}{c|}{0.26}                                 & 67.2                      \\
% PyramidCLIP                        & {\color{ForestGreen}\cmark}                                 & 0.26                        & 0.27                        & \multicolumn{1}{c|}{0.26}                        & {64.3}               & 0.22                        & 0.25                                 & \multicolumn{1}{c|}{0.23}                                 & 70.7         \\
% VQAScore$_\texttt{Gemini Flash}$                        & {\color{ForestGreen}\cmark}                                 & \underline{0.42}                        & \underline{0.54}                       & \multicolumn{1}{c|}{\underline{0.45}}                        & \underline{\textbf{73.1}}               & \underline{0.51}                        & \underline{0.57}                                 & \multicolumn{1}{c|}{\underline{0.49}}                                 & \underline{76.5}                    \\
% {\color[HTML]{9B9B9B} VNLI}        & {\color{red!60} \xmark}          & {\color[HTML]{9B9B9B} 0.37} & {\color[HTML]{9B9B9B} 0.49} & \multicolumn{1}{c|}{{\color[HTML]{9B9B9B} 0.42}} & {\color[HTML]{9B9B9B} 54.4} & {\color[HTML]{9B9B9B} 0.45} & {\color[HTML]{9B9B9B} {0.55}} & \multicolumn{1}{c|}{{\color[HTML]{9B9B9B} {0.45}}} & {\color[HTML]{9B9B9B} 72.7} \\ \hline
% % Gecko+VQAScore$_{\texttt{Gemini Flash}}$                        & \xmark                                 & --                       & --                       & \multicolumn{1}{c|}{--}                        & {81.0}               & --                       & --                                & \multicolumn{1}{c|}{--}                                 & 86.3                                   \\ \hline
% \end{tabular}%
% }
% \caption{\textbf{Correlation between auto-eval metrics and human ratings across annotation templates on Gecko2K.}  With the same backend, \model~outperforms all other QA/VQA metrics across all evaluations and \model~with GeminiFlash performs even better; it performs better or similar to the strongest single-score approach (VQAScore). \small{\textbf{Bold}: Top results. \underline{Underlined}: Top results by category. }}
% \label{tab:corr}}
% % \end{subtable} 
% % \begin{subtable}{.2\linewidth}

%     % \end{minipage} &
    
%     \hfill
%     % \begin{minipage}{.2\linewidth}
    
%     \parbox{.2\textwidth}{
% \centering
% \resizebox{0.2\textwidth}{!}{%
% \begin{tabular}{cccc}
% \toprule                             

%  & WL & \multicolumn{1}{c}{Likert} \\
%  \cmidrule(l){2-3} 
% Metrics & \multicolumn{2}{c}{Pearson} & SxS Acc (\%) \\ 
% \midrule
% VideoCLIP & 0.18 & \multicolumn{1}{c}{0.21} & 28.0 \\
% VQAScore & 0.30 & \multicolumn{1}{c}{0.33} & 52.0 \\
% Gecko$_{\texttt{Gemini Flash}}$ & \textbf{0.43} & \multicolumn{1}{c}{\textbf{0.45}} & \textbf{55.8} \\ 
% \bottomrule
% \end{tabular}%
% % }
% \vspace{3mm}
% \caption{\textbf{Text-to-video: Pearson correlation between VQA-based and contrastive auto-eval metrics and human ratings across annotation templates on VBench overall consistency prompts.} Similar to text-to-image, Gecko again outperforms other auto-eval metrics with higher overall Pearson correlation with absolute ratings and accuracy on side-by-side comparisons demonstrating the generality of the approach to more modalities.}
% }
% \label{tab:corr_pearson_video}}
% % \end{subtable} 

%     % \end{minipage} 
% % \end{tabular}
% \end{table}



\begin{table}[t]
\renewcommand{\arraystretch}{1.1}
\setlength{\tabcolsep}{3pt}
\centering

% \begin{minipage}[b]{0.64\textwidth} % Adjust width as needed

\begin{subtable}[b]{0.69\textwidth}
\centering
\resizebox{\textwidth}{!}{%  <-- Resize to minipage width
\begin{tabular}{c|c|cccc|cccc}
\hline
 & & \multicolumn{4}{c|}{\textbf{Gecko(R)}} & \multicolumn{4}{c}{\textbf{Gecko(S)}} \\ \cline{3-10} 
 & & WL & Likert & DSG(H) & SxS & WL & Likert & DSG(H) & SxS \\ \cline{3-10} 
\multirow{-3}{*}{\textbf{Metrics}} & \multirow{-3}{*}{\textbf{Zero-shot}} & \multicolumn{3}{c|}{SpearmanR} & Acc & \multicolumn{3}{c|}{SpearmanR} & Acc \\ \hline
{\em Interpretable (QA/VQA)} & & & & & & & & & \\
TIFA$_{\texttt{PALM-2/PALI}}$ & {\color{ForestGreen}\cmark} & 0.26 & 0.34 & 0.28 & 41.7 & 0.39 & 0.32 & 0.39 & 53.2 \\
DSG$_{\texttt{PALM-2/PALI}}$ & {\color{ForestGreen}\cmark} & 0.35 & 0.47 & 0.42 & 49.6 & 0.45 & 0.45 & 0.45 & 58.1 \\ 
Gecko$_{\texttt{PALM-2/PALI}}$ & {\color{ForestGreen}\cmark} & \underline{0.41} & \underline{0.55} & \underline{0.46} & \underline{62.1} & \underline{0.47} & \underline{0.52} & \underline{0.45} & \underline{74.6} \\ \hline
Gecko$_{\texttt{Gemini Flash}}$ & {\color{ForestGreen}\cmark} & \underline{\textbf{0.43}} & \underline{\textbf{0.58}} & \underline{\textbf{0.48}} & \underline{72.2} & \underline{\textbf{0.54}} & \underline{\textbf{0.59}} & \underline{\textbf{0.56}} & \underline{\textbf{78.8}} \\ \hline
{\em Uninterpretable (single score)} & & & & & & & & & \\
CLIP & {\color{ForestGreen}\cmark} & 0.14 & 0.16 & 0.13 & 54.4 & 0.25 & 0.18 & 0.26 & 67.2 \\
PyramidCLIP & {\color{ForestGreen}\cmark} & 0.26 & 0.27 & 0.26 & 64.3 & 0.22 & 0.25 & 0.23 & 70.7 \\
VQAScore$_\texttt{Gemini Flash}$ & {\color{ForestGreen}\cmark} & \underline{0.42} & \underline{0.54} & \underline{0.45} & \underline{\textbf{73.1}} & \underline{0.51} & \underline{0.57} & \underline{0.49} & \underline{76.5} \\
{\color[HTML]{9B9B9B} VNLI} & {\color{red!60} \xmark} & {\color[HTML]{9B9B9B} 0.37} & {\color[HTML]{9B9B9B} 0.49} & {\color[HTML]{9B9B9B} 0.42} & {\color[HTML]{9B9B9B} 54.4} & {\color[HTML]{9B9B9B} 0.45} & {\color[HTML]{9B9B9B} 0.55} & {\color[HTML]{9B9B9B} 0.45} & {\color[HTML]{9B9B9B} 72.7} \\ \hline
\end{tabular}%
}
\caption{\textbf{Correlation between auto-eval metrics and human ratings across annotation templates on Gecko2K.}  With the same backend, \model~outperforms all other QA/VQA metrics across all evaluations and \model~with GeminiFlash performs even better; it performs better or similar to the strongest single-score approach (VQAScore). \small{\textbf{Bold}: Top results. \underline{Underlined}: Top results by category. }}
\label{tab:corr}
\end{subtable}
\hfill
\begin{subtable}[b]{0.3\textwidth}
% \begin{minipage}[b]{0.34\textwidth} % Adjust width as needed
\centering
\resizebox{\textwidth}{!}{%  <-- Resize to minipage width
\begin{tabular}{cccc}
\toprule                             
 & WL & Likert \\  \cmidrule(l){2-3}  % Corrected cmidrule
Metrics & \multicolumn{2}{c}{Pearson} & SxS Acc (\%) \\ 
\midrule
VideoCLIP & 0.18 & 0.21 & 28.0 \\
VQAScore$_{\texttt{Gemini Flash}}$ & 0.30 & 0.33 & 52.0 \\
Gecko$_{\texttt{Gemini Flash}}$ & \textbf{0.43} & \textbf{0.45} & \textbf{55.8} \\ 
\bottomrule
\end{tabular}%
}
\caption{\textbf{Pearson correlation between auto-eval metrics and human ratings on VBench for text-to-video evaluation.} Gecko outperforms all other metrics across human templates demonstrating the generality of the approach to more modalities.}
\label{tab:corr_pearson_video}
\end{subtable}
% \end{minipage}
\end{table}

==> tables/correlation_pearson_video.tex <==
\begin{table}[t]
\renewcommand{\arraystretch}{1.2}
\setlength{\tabcolsep}{3pt}

\centering
% \resizebox{\textwidth}{!}{%
\begin{tabular}{cccc}
\toprule                             
{\multirow{2}{*}{\textbf{Metrics}}}
 & \multicolumn{1}{c}{WL} & \multicolumn{1}{c}{Likert} & \multicolumn{1}{c}{SxS} \\
 & \multicolumn{2}{c}{Pearson} &  Acc \\ 
\midrule
VideoCLIP & 0.18 & \multicolumn{1}{c}{0.21} & 28.0 \\
VQAScore$_{\texttt{Gemini Flash}}$ & 0.30 & \multicolumn{1}{c}{0.33} & 52.0 \\
Gecko$_{\texttt{Gemini Flash}}$ & \textbf{0.43} & \multicolumn{1}{c}{\textbf{0.45}} & \textbf{55.8} \\ 
\bottomrule
\end{tabular}%
% }
\vspace{3mm}
\caption{\textbf{Text-to-video: Pearson correlation between VQA-based and contrastive auto-eval metrics and human ratings across annotation templates on VBench overall consistency prompts.} Similar to text-to-image, Gecko again outperforms other auto-eval metrics with higher overall Pearson correlation with absolute ratings and accuracy on side-by-side comparisons demonstrating the generality of the approach to more modalities.}
\label{tab:corr_pearson_video}
% \vspace{-5mm}
\end{table}

==> tables/human_eval_krippendorffs.tex <==
\begin{table}[h]
\centering
\resizebox{0.5\textwidth}{!}{
\begin{tabular}{c|ccc|ccc}
\hline
\multirow{2}{*}{Gen. model} & \multicolumn{3}{c|}{\textbf{Gecko (R)}} & \multicolumn{3}{c}{\textbf{Gecko (S)}} \\ \cline{2-7} 
                            & Likert         & WL          & DSG (H)         & Likert      & WL       & DSG (H)      \\ \hline
SD 1.5                      & 0.36          & $\mathbf{0.66}         & $\mathbf{0.66}$          & 0.59       & 0.69      & $\mathbf{0.74}$       \\
SD XL                       & $\mathbf{0.76}          & 0.75         & 0.57          & 0.54       & 0.67      & 0.70       \\
Muse 2.3                    & 0.78          & $\mathbf{0.82}         & 0.72          & 0.58       & 0.69      & 0.72       \\
Imagen 2.5                  & 0.64          & $\mathbf{0.81}         & 0.68          & 0.57       & 0.72      & 0.75       \\ \hline
\end{tabular}}
\caption{Measuring inter-rater agreement for each human evaluation template with Krippendorff's $\alpha$. Higher values indicate better agreement. \todo{two floating points}
\su{what does boldface indicate here?}
}
\label{tab:h_eval_krippendorffs}
\end{table}

==> tables/human_eval_model_comparison_with_p_val.tex <==

\begin{table}[]
\centering
\resizebox{0.5\textwidth}{!}{
\begin{tabular}{c|ccc|ccc}
\hline
                   & \multicolumn{3}{c|}{\textbf{Gecko (R)}}                                                                                                                                     & \multicolumn{3}{c}{\textbf{Gecko (S)}}                                                                                                                                                                             \\ \cline{2-7} 
\multirow{-2}{*}{} & Muse 2.3                                   & SD XL                                             & SD 1.5                                                         & Muse 2.3                                                       & SD XL                                                                & SD 1.5                                                               \\ \hline
Imagen 2.5             & \cellcolor[HTML]{FFFFC7}<{},=,= & \cellcolor[HTML]{FFFFC7}<{},<{},= & \cellcolor[HTML]{FFFFC7}<{},<{},>{} & \cellcolor[HTML]{D4FFD3}<{},<{},<{} & \cellcolor[HTML]{D4FFD3}=,=,=                                        & \cellcolor[HTML]{D4FFD3}>{},>{},>{} \\
Muse 2.3               & x                                       & \cellcolor[HTML]{FFFFC7}=,<{},=           & \cellcolor[HTML]{FFFFC7}=,>{},>{}        & x                                                           & \cellcolor[HTML]{D4FFD3}>{},>{},>{} & \cellcolor[HTML]{D4FFD3}>{},>{},>{} \\
SD XL              & x                                       & x                                                 & \cellcolor[HTML]{FFFFC7}>{},=,>{}        & x                                                           & x                                                                    & \cellcolor[HTML]{D4FFD3}>{},>{},>{} \\ \hline
\end{tabular}}
\caption{\textbf{Comparing models using human annotations.} We perform the Wilcoxon signed-rank test for all pairs of models (p<0.001) and post-hoc comparison based on the average ratings (Table \ref{tab:h_eval_avg_std}). For each entry of the table, the symbols sequence represents the result of WL, Likert, and DSG (H), respectively. Each symbol indicates whether the model in the row was significantly better (>), worse (<), or not significantly different (=) than the model in the column. \todo{prettify}}
\label{tab:h_eval_wilcoxon}
\end{table}

==> tables/human_eval_model_comparison_with_p_val_rel_prompts.tex <==
\begin{table}[]
\centering
\resizebox{0.5\textwidth}{!}{
\begin{tabular}{c|ccc|ccc}
\hline
                 & \multicolumn{3}{c|}{\textbf{Gecko (R)}}            & \multicolumn{3}{c}{\textbf{Gecko (S)}}                                                                                                                                                                             \\ \cline{2-7} 
\multirow{-2}{*}{} & Muse 2.3                                   & SD XL                                             & SD 1.5                                                         & Muse 2.3                                                        & SD XL                                                                & SD 1.5                                                               \\ \hline
Imagen 2.5            & \cellcolor[HTML]{FFFFC7}<,<,= & \cellcolor[HTML]{FFFFC7}<,<,> & \cellcolor[HTML]{FFFFC7}<,<,> & \cellcolor[HTML]{D4FFD3}<,<,< & \cellcolor[HTML]{D4FFD3}=,=,=  & \cellcolor[HTML]{D4FFD3}>,>,> \\
Muse 2.3              & x                                       & \cellcolor[HTML]{FFFFC7}=,=,<           & \cellcolor[HTML]{FFFFC7}>,=,>        & x                                                           & \cellcolor[HTML]{D4FFD3}>,>,> & \cellcolor[HTML]{D4FFD3}>,>,> \\
SD XL              & x                                       & x                                                 & \cellcolor[HTML]{FFFFC7}=,=,>        & x                                                           & x                                                                    & \cellcolor[HTML]{D4FFD3}>,>,> \\ \hline
\end{tabular}}
\caption{\textbf{Reliable prompts - Pairwise comparison of models across the three absolute comparison templates.} }
\end{table}
